Generating Faithful and Complete Hospital-Course Summaries from the Electronic Health Record

The rapid adoption of Electronic Health Records (EHRs) has been instrumental in streamlining administrative tasks, increasing transparency, and enabling continuity of care across providers. An unintended consequence of the increased documentation burden, however, has been reduced face-time with patients and, concomitantly, a dramatic rise in clinician burnout. In this thesis, we pinpoint a particularly time-intensive, yet critical, documentation task: generating a summary of a patient's hospital admissions, and propose and evaluate automated solutions. In Chapter 2, we construct a dataset based on 109,000 hospitalizations (2M source notes) and perform exploratory analyses to motivate future work on modeling and evaluation [NAACL 2021]. In Chapter 3, we address faithfulness from a modeling perspective by revising noisy references [EMNLP 2022] and, to reduce the reliance on references, directly calibrating model outputs to metrics [ACL 2023]. These works relied heavily on automatic metrics as human annotations were limited. To fill this gap, in Chapter 4, we conduct a fine-grained expert annotation of system errors in order to meta-evaluate existing metrics and better understand task-specific issues of domain adaptation and source-summary alignments. To learn a metric less correlated to extractiveness (copy-and-paste), we derive noisy faithfulness labels from an ensemble of existing metrics and train a faithfulness classifier on these pseudo labels [MLHC 2023]. Finally, in Chapter 5, we demonstrate that fine-tuned LLMs (Mistral and Zephyr) are highly prone to entity hallucinations and cover fewer salient entities. We improve both coverage and faithfulness by performing sentence-level entity planning based on a set of pre-computed salient entities from the source text, which extends our work on entity-guided news summarization [ACL, 2023], [EMNLP, 2023].

==> Preface.tex <==
%Preface page. 
%This page is optional


\begin{center}
\vspace*{5\baselineskip}
\textbf{\large Introduction or Preface}
\end{center}


\begin{flushleft}
\hspace{10mm}Insert your preface text here if applicable. This page is optional, you may delete it if not needed. If you delete this page make sure to move page counter comment in thesis.tex to correct location. 
\end{flushleft}


%\pagenumbering{gobble}  %remove page number on summary page




==> approvalPage.tex <==


\newcommand{\CopyrightYear}{2019}


\begin{titlepage}
\begin{singlespacing}
\begin{center}

\vspace*{35\baselineskip}

Symbol \CopyrightYear\\
\vspace{\baselineskip}	
[Author Name]\\
\vspace{\baselineskip}	
All Rights Reserved
\end{center}
\vfill

\end{singlespacing}
\end{titlepage}


==> revision_tables/training_sets_table.tex <==
\begin{table*}[t]
% keep : Train #, tokens, entities, hallucination, source recall
\centering
\footnotesize 
\begin{tabular}{cc|ccccc}
\textbf{Reference} & \textbf{Quality} & \textbf{\# Training} & & & \multicolumn{2}{c}{\textbf{Entity-Level Source Overlap}} \\
\textbf{Version} & \textbf{Strategy} & \textbf{Examples} & \textbf{Avg. \# Tokens} & \textbf{Avg. \# Entities} & \textbf{Avg. Precision}& \textbf{Avg. Recall} \\ \hline
\textbf{Original} & Original & 45k & 370 & 50 & 60.4 & 26.8 \\
\hline
\multirow{2}{*}{\textbf{Filtered}} & No Admission & 5.7k & 420 & 64 & 91.5 & 32.7 \\
 & Unsupported & 6.0k & 381 & 55 & 95.7 & 28.9 \\  \hline
\multirow{3}{*}{\textbf{\makecell{Revised\\(Ours)}}} & Fully Extractive & 45k & 295 & 28 & 100 & 19.6 \\
 & Less Abstractive & 45k & 300 & 29 & 97.6 & 36.8 \\
 & More Abstractive & 45k & 272 & 26 & 96.8 & 35.0  \\ \hline
\end{tabular}
\caption{Training datasets obtained from the revision strategies according to size (number of references), average number of tokens and entities in the references, and entity-level overlap with sources (average precision and recall).} 
% 85.7, 84.0, 83.3
%Revised training data. \textbf{Faithfulness} is precision-oriented, with \textbf{BS Prec} (BERTScore precision) and \textbf{Halluc.} (hallucination rate) computed vis-a-vis the source notes. \textbf{Entity Coverage} is recall-oriented, broken down by fraction of (supported) entities included from the original reference (\textbf{Ref.}), and separately, the source (\textbf{Source}).}
\label{tab:revision}
\end{table*}


==> revision_tables/transfer_table.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{l|ccc}
\textbf{Pretrain Dataset} & \textbf{R1} & \textbf{R2} & \textbf{RL} \\ \hline
\textbf{Original} & 27.25 & 8.61 & 16.25 \\
\textbf{Filtered - Unsupported} & 25.68 & 6.74 & 14.97 \\
\textbf{Filtered - Loss Truncation} & 27.15 & 8.24 & 15.98 \\
\textbf{Control - Hallucination} & 27.55 & \textbf{8.73} & 16.36 \\
\textbf{Revised - Fully Extractive} & 26.29 & 7.71 & 15.34 \\
\textbf{Revised - Less Abstractive} & 27.71 & 8.66 & 16.23 \\
\textbf{Revised - More Abstractive} & \textbf{27.73} & \textbf{8.73} & \textbf{16.42} \\
\end{tabular}
\caption{Zero-Shot performance on unseen hospital-course corpus for models pre-trained on original, filtered, and revised MIMIC-III references. \textbf{Best bolded}.} %  The LongFormer models are shown.
\label{tab:results-transfer}
\end{table}

